Multilingual Machine Translation Systems from Microsoft for WMT21 Shared Task

This report describes Microsoft's machine translation systems for the WMT21 shared task on large-scale multilingual machine translation. We participated in all three evaluation tracks including Large Track and two Small Tracks where the former one is unconstrained and the latter two are fully constrained. Our model submissions to the shared task were initialized with DeltaLM\footnote{\url{https://aka.ms/deltalm}}, a generic pre-trained multilingual encoder-decoder model, and fine-tuned correspondingly with the vast collected parallel data and allowed data sources according to track settings, together with applying progressive learning and iterative back-translation approaches to further improve the performance. Our final submissions ranked first on three tracks in terms of the automatic evaluation metric.

==> model.tex <==
% \section{Background}

% Multilingual Neural Machine Translation (MNMT),
% which leverages a single system to handle multiple languages at once, has drawn research attention in recent years. It has shown great potential to transfer knowledge form high-resource languages to low-resource languages. MNMT is a powerful paradigm to  reduce the cost of training
% and serving separate models for different language
% pairs. 

% Collecting
% high-quality data suitable for the evaluation MNMT process
% is difficult in low-resource scenarios. \citet{flores_101} present a benchmark dataset FLORES-101, which contains high-quality and high-coverage of low-resource languages to evaluate how well the methods' generalize and scale to a larger number of languages with diversity of linguistic features. The total dataset translates 3001 sentences into 101 languages. It is non-trivial to build such benchmark, because the scarce availability for low-resource languages is obvious and can not check their quality. 
%%
%why mutlilingual MT

% To go a step further to bring the community together on the topic of low-resource multilingual machine translation, WMT21 shared task on large-scale multilingual machine translation introduced a realistic benchmark with 3 tracks to foster progress of evaluating of many-to-many multilingual translation. Shared tasks can be divided into three tracks: Large Track, Small Track \#1 and Small Track \#2. Two small track are to evaluate the translation quality of low-resource languages with English from two language families: Central/East European and South East Asian. It does not require large computational resources at training time. But the large track is to translate more than 10,302 language pairs at once,
% it not only requires a substantial amount of training time for a very large number of languages, but also ensures the system could translate 102 languages on test case in a limited time. We present dataset details of three tracks in section 4.2.

%结构初始化

% We are going to have three tracks: two small tasks and a large task.
% The small tracks evaluate translation between fairly related languages and English (all pairs). The large track uses 101 languages.

% The small tracks are an example of a practical MMT problem in similar languages, which does not require very large computational resources at training time, particularly so given the pretrained models we provide.

% At the other end of the spectrum, the large track explores the very ambitious goal to translate all at once a very large number of languages which may require a substantial amount of compute at training time

% . The small tracks evaluate translation between fairly related languages and English (all pairs). The large track uses 101 languages. The goal of these tasks is to alleviate the challenge of low-resource multilingual machine translation by leveraging single large-scale multilingual model.

% Track
% For small tracks, it does not require very large computational resources at training time.
% The small track #1 consists in 5 Central/East European languages, 30 directions: Croatian, Hungarian, Estonian, Serbian, Macedonian, English. The small track #2 is using 5 South East Asian languages, 30 directions: Javanese, Indonesian, Malay, Tagalog, Tamil, English. A multilingual machine translation system may be capable of translating a sentence into several languages, or to translate sentences from several languages into a given language or any combinations thereof. Participation was  constrained for the small tasks, where only the data available in these tasks is allowed. Pre-trained models are OK to use as long as they are publicly available for download. The goal aimed at fostering work on improving the translation quality of low-resource language pairs by leveraging from multiple languages.

% Over recent years, the main translation task at WMT has challenged participants with low-resource languages limited to a handful of languages. These tasks have only considered translation English only, while the recent work has been focusing on large-scale multilingual to solve low-resource languages ~\cite{m2m,freitag2020complete}. Hence,
% the full track: FLORES-101 presented a large-scale many-to-many dataset, coverage of high-quality low resource languages, it forces the model to translate more than 10,100 language pairs. For allowed resources, the large track is fully unconstrained on model and training data.



\section{Models}

Our multilingual translation systems are built upon DeltaLM~\cite{deltalm}, a public available pretrained language model.
We fine-tune the model for Large track, Small track \#1, and Small track \#2 respectively following the same process. 
To benefit from a deeper encoder, we apply progressive learning to train a 24 encoder and 12 decoder model firstly and then continue-train it by adding 12 layers on the top of the encoder.
To further improve the performance, we also construct parallel back-translation data with iterative back-translation~\cite{iterative_bt} and implement the pivot translation~\cite{pivot_based_transfer_learning} for some translation directions.

% \begin{figure*}[t]
% \begin{center}
% 	\includegraphics[width=1.0\textwidth]{graph/M4_Model.pdf}
% 	\caption{The model architecture used to perform on WMT21 shared task for large-scale multilingual machine translation. We first train a model with 24 encoder layers and 12 decoder layers by initializing with DeltaLM checkpoint, and then continue-train it by adding 12 layers on the top of the encoder.}
% 	\label{pipeline_m4}
% \end{center}
% \end{figure*}

% In the following section, we will first compare the pre-trained model DeltaLM with M2M~\cite{m2m}, how we initialize and expand the model, and iterative  back-translation ~\cite{iterative_bt} of multiple rounds and pivot translation to alleviate low-resource issues.

\subsection{Fine-tuning from DeltaLM}

Our system apply multilingual pretrained DeltaLM~\cite{deltalm} to initialize encoder-decoder architecture and consistent sentencepiece ~\cite{spm}. We also follow the heuristic data-sampling strategy with temperature-based batch balancing ~\cite{m2m,zcode} to ease underrepresented of low-resource languages. The probability of picking language is proportional to its number of sentences,$D_l$,i.e., $p_l=\frac{D_l}{\sum_i{D}_i}$. And set temperature $T=5$ to rescale and control the distribution $p_l^\frac{1}{T}$, especially for low-resource languages.



\paragraph{DeltaLM}

DeltaLM is a multilingual pretrained encoder-decoder model, which has been proven useful for multilingual machine translation. It pretrained with span corruption~\cite{mt5} and translation span corruption~\cite{mt6} tasks by leveraging both large-scale monolingual data
and bilingual data.
%architecture
Different from the prior encoder-decoder architecture, DeltaLM introduced an interleaved decoder that has a more consistent structure
with the encoder. It interleaves FFNs modules at decoder to make the structure more consistent with encoder. Therefore, each decoder block
consists of one self-attention, one cross-attention,
and two FFNs. 
%Initialized
% DeltaLM uses InfoXLM~\cite{chi2020infoxlm}  as pre-trained weight, which proposes a novel cross-lingual contrast to enhance
% the cross-lingual transferability.
% To fully use the pretrained InfoXLM
% weights and make none of the sub-layer randomly initialized, DeltaLM
% divides the decoder block into two parts for initialization. For the self-attentions and the bottom FFNs of each decoder block, it initializes with the odd layers of InfoXLM. Cross-attentions
% and the top FFNs of each decoder block are initialized with the corresponding even layers of pretrained encoder. The rest components are maintained with the same weight from InfoXLM, such as embeddings, residual connections, the activation function, and the layer normalizations.


% initializes the bottom part of each decoder block: the self-attentions and the bottom FFNs, based on odd layers of pre-trained InfoXLM, and the top part of eh the different layers of encoder: self-attention-FFN and the first half: cross-attention-FFN
% With the interleaved structure, the decoder and encoder can be directly initialized  with the pretrained encoder InfoXLM~\cite{chi2020infoxlm}. 
% To fully use the pretrained InfoXLM
% weights and make none of the sub-layer randomly initialized, DeltaLM initializes
% the self-attentions and the bottom FFNs with the
% odd layers of InfoXLM, while the cross-attentions
% and the top FFNs are initialized with the corresponding even layers. The rest components also initializes with the same weight from pretrained InfoXLM, such as embeddings, residual connections, the activation function, and the layer normalizations.


% For DeltaLM encoder, DeltaLM applies pre-trained encoder InfoXLM~\cite{chi2020infoxlm} as initilized weight. 
% This encoder training with large-scale monolingual
% data and bilingual data through three pre-training tasks: masked language model, translation language model and cross-lingual constract objectives.
% Specailly, DeltaLM makes the decoder structure more consistent with encoder and none of the sub-layer will be randomly initialized. It replaces each block of odd layer with one self-attention, one cross-attention, and two FFNs. For initialized decoder, DeltaLM initialized
% the self-attentions and the bottom FFNs with the
% odd layers of InfoXLM, while the cross-attentions
% and the top FFNs are initialized with the corresponding even layers. 
% The rest components of the decoder, including the
% embeddings, residual connections, the activation
% function, and the layer normalizations, are the same
% as the pretrained encoder. After initilized encoder and decoder, DeltaLM pre-trains with two tasks: span corruption ~\cite{raffel2019exploring}
% and translation span corruption ~\cite{chi2020infoxlm}.

\paragraph{Progressive Training}

To explore the effects of DeltaLM for multilingual machine translation, we present a new progressive learning to initialize our model. The training process can be divided into two stages: 1) the first stage is that applies DeltaLM 24-layer encoder and 12-layer decoder structure, in which both the encoder and decoder are initialized by InfoXLM. It can directly use the checkpoint of DeltaLM for initializing and leveraging the knowledge from pre-training corpus to guide system to understand some language pairs covered by WMT21 shared task and pre-training corpus. 2) The shallow translation model with the 24 encoder layers and 12 decoder layers initialized by the DeltaLM is finetuned on the multilingual corpora 3) to scale the model to understand the diversity of linguistic features with more additional languages, we further increase the depth of the encoder to the 36 layers based on the shallow translation model with the 24 encoder layers. This stage will continue training the model by adding 12 layers on the top of the encoder. Although the additional 12 layers of encoder are initialized randomly in the second stage, it can also improve the capacity of understanding linguistic phenomena 
for large number of languages, especially low-resource languages.




% We train both the small track #1, the small track #2 and the full track. Our model is based on pretrained DeltaLM ~\cite{deltalm}. We perform fine-tuning in these three Many-to-Many tasks respectively as our base model. To improve the translation directions for all languages, we additionally construct parallel back-translation corpus, where the training data of any two languages are parallel and translated from the same monolingual English data. We leverage the Microsoft translator, M2M \cite{m2m}, and our multilingual model to translate the Wikipedia English monolingual sentences.
% For these synthetic bilingual data, we experiment
% with dynamic data sampling to estimate the optimal way to feed the model these synthetic bilingual data for alleviating data imbalance across
% different languages. Training the model with the
% true data distribution would starve the low-resource
% language pairs. Some low-resource corpus is very difficult to obtain, so we have adopted the hybrid pivot strategy, and leverage high quality English to transfer knowledge for low-resource languages. 




% \subsection{Mutlilingual Pre-trained Model}

% Most of machine translation models are based on the encoder-decoder structure, so the pretrained encoders can efficiently obtain knowledge to improve the machine translation quality. Some encoder-decoder architecture, such as BART ~\cite{lewis2019bart} and T5 ~\cite{raffel2019exploring},
% explore self-supervised tasks to efficiently
% pre-train the models from scratch. Motivated by M2M \cite{m2m} and DeltaLM ~\cite{deltalm} which can support many-to-many translation and also efficiently initialize decoder for downstream task. We initialize our systems with an encoder-decoder Transformer ~\cite{vaswani2017attention}, which
% is pretrained using the DeltaLM weight. In this section, we will give brief details about M2M and DeltaLM, and how to adapt DeltaLM to FLORES-101 tasks. 

% \paragraph{M2M}

% M2M ~\cite{m2m} creates a large-scale Many-to-Many dataset for 100 languages. It applies automatic construction with mining strategy to exploit parallel corpora ~\cite{schwenk2019ccmatrix}. M2M also leverages back-translation to enhance the translation quality. Totally, M2M trains 100 languages of 7.5B training sentences to support Many-to-Many translation directions. To make sure neural networks with standard capacity can learn this Many-to-Many dataset with increasing number of languages. M2M also leverages in scaling ~\cite{kaplan2020scaling,huang2019gpipe} the capacity of models and train them efficiently. It can scale the models
% that are over 50 times larger than current bilingual models with model parallelism.

% The M2M-100 ~\cite{m2m} model does not have full
% coverage of the languages in FLORES-101. Hence the FLORES-101 ~\cite{flores_101} extended from OPUS for some low-resource languages, thus obtained 124 languages. This work presented two different sizes of models: 615M and 175 parameters.


% \paragraph{DeltaLM}
% DeltaLM ~\cite{deltalm} is a pretrained multilingual encoder-decoder
% model, which initialized encoder and decoder at the same time and fully leverage  through multilingual encoder. 

% For DeltaLM encoder, DeltaLM applies pre-trained encoder InfoXLM~\cite{chi2020infoxlm} as initilized weight. This encoder training with large-scale monolingual
% data and bilingual data through three pre-training tasks: masked language model, translation language model and cross-lingual constract objectives.

% To solve the encoder can be directly initialized with
% the pretrained multilingual encoder, but it is non-trivial
% to initialize the decoder. DeltaLM makes the decoder structure more consistent with encoder and none of the sub-layer will be randomly initialized. It replaces each block of  odd layer with one self-attention, one cross-attention,and two FFNs. For initialized decoder, DeltaLM initialized
% the self-attentions and the bottom FFNs with the
% odd layers of InfoXLM, while the cross-attentions
% and the top FFNs are initialized with the corresponding even layers. 
% The rest components of the decoder, including the
% embeddings, residual connections, the activation
% function, and the layer normalizations, are the same
% as the pretrained encoder. After initilized encoder and decoder, DeltaLM pre-trains with two tasks: span corruption ~\cite{raffel2019exploring}
% and translation span corruption ~\cite{chi2020infoxlm}. Therefore, we can simply initialize the encoder and decoder at the same time  to perform many-to-many translation tasks.

% %突出deltalm 扩展到36层 encoder
% In particular, considering the model performance and inference time, we further increase the depth of the encoder to the 36 layers for better performance. We initialized the first 24 layers of encoder with DeltalLM weight, and the last 12 layers were initialized randomly. We think larger models have better capacity to understand low resource language.


% X Y any non english 
\subsection{Data Augmentation}
% \subsection{Offline Iterative Back-translation}
Considering some training data in low-resource languages are scarce, we perform iterative back-translation ~\cite{iterative_bt} to ease the problem. We set the model trained Many-to-Many translation in the previous subsection as base model. To generating high quality back translation (BT) data, we combine  M2M ~\cite{m2m}, in-house Translator and base model to determine a more meaningful way.
For the BT data in the X$\to$En and En$\to$X directions, we compared the performance on three different systems and generated the corresponding X based on the English of the wiki.
For the BT data in the X$\to$Y direction (Any language pairs without English involved), we adopted a heuristic method. It could translate En$\to$X and En$\to$Y from same English monolingual text, and then use (X, Y) as generated BT data. If there is enough monolingual text in X or Y, our system can still directly translate in X$\to$Y direction or Y$\to$X to obtain BT data.

In order to further improve the performance of low-resource language pairs on X$\to$Y direction, we adopt pivot translation ~\cite{pivot_based_transfer_learning} to improve translation quality. Most of our pivot language in the X$\to$Y direction is English, but if the performance of  X$\to$Y on dev is better than pivot translation X$\to$En$\to$Y, we directly apply X$\to$Y for the language pair.

% Due to the limits of time and GPU memories of the shared task, we do not explore other approaches like mixture-of-experts (MOE) and model ensemble.

% If the model performs better on X$\to$En and En$\to$Y and the data on X$\to$Y is scarce, then we will use pivot language localization sequence: X $\to$ Pivot (bridge) language $\to$ Y.
% Pivot Translation has been proven to greatly improve the performance of X$\to$Y language pairs, especially when corpus is scarce.
% There is also a part of X$\to$Y that is maintained in the original training set without pivot. So it is a hybrid pivot translation.
% Considering mistranslation in the pivot language reproduced in the target languages and lacking some linguistic markers that the source and target languages might have, 

% we do not use English as pivot translation for all X$\to$Y. If the model performs better on X$\to$E and E$\to$Y and the data on X$\to$Y is scarce, then we will use pivot language localization sequence: X $\to$ Pivot (bridge) language $\to$ Y.
% Most of our pivot language in the X$\to$Y direction use English as the pivot language. But considering some collected high-quality X$\to$C, C$\to$Y training data, we still use non-English pivot languages such as Chinese.

% Due to the limits of time and GPU memories of the shared task, we do not explore other approaches like mixture-of-experts (MOE) and model ensemble.


% We also experiment with creating synthetic training data using  back-translation with one MNMT model. We assumed that our base MNMT model
% is of reasonable quality. At the same time, the performance of different systems is also different, so we combine M2M, Microsoft Translator and our base MNMT model to generate back translation data and conduct experiments to determine a more meaningful way.
%
% First of all, for the bilingual data in the X$\to$E and E$\to$X directions, we compared the performance on three different systems, selected the best model and generated the corresponding X based on the English of the wiki.
%
% Due to the scarcity of data in the X$\to$Y direction and the uneven quality of FLORES-101, we adopted a heuristic method to generate X$\to$Y back-translation data. Our method can be divided into three categories: 1) We employ MNMT model to translate E$\to$X and E$\to$Y from same English monolingual text, and then use <X, Y> as generated BT data, 2) Regardless of the depending on English, our MNMT model can still directly translate the X$\to$Y direction. Therefore, we use the model to generate Y1 and Y2 for the monolingual X.
% 3) For monolingual X, we translate from X$\to$Y direction to obtain pseudo <X,Y> bitext.

% \subsection{Hybrid Pivot Translation for Low-resource Languages}














